A Taxonomy of Challenges to Curating Fair Datasets

Despite extensive efforts to create fairer machine learning (ML) datasets, there remains a limited understanding of the practical aspects of dataset curation. Drawing from interviews with 30 ML dataset curators, we present a comprehensive taxonomy of the challenges and trade-offs encountered throughout the dataset curation lifecycle. Our findings underscore overarching issues within the broader fairness landscape that impact data curation. We conclude with recommendations aimed at fostering systemic changes to better facilitate fair dataset curation practices.

==> Input/checklist.tex <==
%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%



\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{Refer to~\Cref{sec:limitations}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{Refer to~\Cref{impact}.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
     \answerNA{}
	\item Did you include complete proofs of all theoretical results?
     \answerNA{}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNA{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
     \answerNA{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
     \answerNA{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
     \answerNA{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
     \answerNA{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
   \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerYes{Refer to~\Cref{methods}. We provide the interview protocol.}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerYes{Refer to~\Cref{methods}. Our study was approved by Arizona State University's Institutional Review Board.}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerYes{Refer to~\Cref{methods}. Compensation consisted of a \$75 Amazon gift card, or the equivalent in the participant's local currency. In total, \$2,250 was spent on participant compensation.}
\end{enumerate}



==> Input/old-background.tex <==
% \section{Background}

% One of the central concerns underscoring the pursuit of fair ML remains the datasets used to develop ML systems ~\cite{paullada2021data,birhane2021large,birhane2021multimodal,buolamwini2018gender,luccioni2021s}. Yet obtaining fair and ethically-sourced datasets remains a challenge. Current large-scale datasets used for training and evaluating ML systems have been plagued with ethical issues, such as the presence of harmful and offensive content~\cite{birhane2021large,crawford2021excavating,zhao2021understanding}, inadequate representation of historically marginalized communities~\cite{buolamwini2018gender,hirota2022gender,garcia2023uncurated}, and the reinforcement of negative stereotypes~\cite{birhane2021multimodal,crawford2021excavating,paullada2021data}. Dataset annotations can  introduce unwanted biases into datasets and replicate socially dominant viewpoints~\citep{miceli2020between}, often stemming from the instructions provided to annotators~\cite{parmar2023don} or annotators' social identities~\cite{ding2022impact,al2020identifying,sap2022annotators,liu2022toward}. Ethical concerns extend beyond representations embedded into the data itself, to the methodologies used for data acquisition, which, in certain instances, mirror colonialist attitudes by being conducted without the consent or participation of human data subjects~\cite{andrews2023ethical,birhane2021large,peng2021mitigating,scheuerman2021datasets}. These nonconsensual practices treat personal data as mere ``raw material''~\cite{birhane2020algorithmic}. Some assert that consent holds a critical role as it serves as the final safeguard for individuals against the potential misuse of their personal information, especially when it conflicts with their interests or well-being~\cite{mittelstadt2016ethics,de2016new,politou2018forgetting,paullada2021data}. Importantly, gathering data without obtaining informed consent poses an obstacle for researchers and practitioners in comprehending and mitigating potential harms to data subjects~\cite{van2020ethical,metcalf2016human}.  When biased datasets are used for training and evaluating ML technologies, they can lead to unfair systems~\cite{parkhi2015deep,guo2016ms,kemelmacher2016megaface,merler2019diversity,torralba200880,deng2009imagenet} or those relying on spurious correlations~\cite{hendricks2018women,menon2020pulse,hill2020wrongfully,barr2015google,sagawa2019distributionally,geirhos2020shortcut,beery2018recognition,rosenfeld2018elephant}. They have the potential to perpetuate and exacerbate existing biases, where certain groups are unfairly allocated or denied opportunities and resources, such as the right to safety, nondiscrimination, and equal treatment (e.g., \cite{wilson2019predictive, papakyriakopoulos2023augmented, norori2021addressing}.

% Efforts within HCI, ML, and data science have sought to address some of these fairness and privacy concerns by rectifying issues in existing datasets. For instance,~\citet{yang2020towards}'s updates on ImageNet removed offensive and non-imageable categories from the dataset's taxonomy. However, datasets, such as ImageNet, initially conceived without explicit fairness considerations, may still prove insufficient for revealing or mitigating bias. For example, this kind of data (collected without participation) often lacks self-identified annotations from data subjects, which are essential to fairness assessments. Therefore, researchers and practitioners have resorted to human annotators to infer data subject characteristics. However, when these inferences are incorrect, they can induce psychological harm~\cite{campbell2007implications,roth2016multiple} and compromise the validity of research, policy, and decision-making~\citep{wang2021fair,cooper2021emergent,richardson2019dirty,andrus2020working}. Furthermore, depending on the domain and context, obtaining sensitive information presents challenges, such as historical mistrust in clinical research among African-Americans~\citep{eyal2014using,lee2021included} or the social stigma of being photographed that some women face~\citep{jo2020lessons}. Marginalized communities may require explicit explanations and assurances about data usage to address concerns related to service provision, security, allocation, and representation~\citep{xiang2022being}.

% Given the integral issues underlying existing datasets, many researchers have advocated for the creation of entirely new ones~\cite{alvi2018turning,buolamwini2018gender,karkkainen2021fairface,merler2019diversity,ramaswamy2023beyond,wang2020mitigating}, e.g., using consent-driven, participatory approaches to data collection~\cite{hazirbas2021towards, porgali2023casual, rojas2022the, ramaswamy2023geode, grauman2022ego4d}. However, collecting ``fairness-aware'' datasets has its limitations and challenges. While still a growing area of research, prior studies on ML practitioners have found that defining identity-related categories for fairness purposes is difficult \cite{}, particularly when practitioners do not inhabit the identities of affected populations \cite{}, and that there is confusion regarding what information should be collected from data subjects~\citep{holstein2019improving}. Everything from regulatory bodies, conflicting stakeholder goals, and epistemic differences influence the curation of datasets \cite{}. Further, dataset practices are often not prioritized in either academic or industrial settings \cite{scheuerman2021datasets}, meaning practitioners are faced with time and resource constraints that promote reactive rather than proactive fairness practices \cite{}. 

% While prior work has contributed great strides to the development of best practices for responsible dataset collection (e.g., dataset documentation~\cite{gebru2018datasheets,bender2018data,pushkarna2022data,papakyriakopoulos2023augmented,heintz2023datasheets,srinivasan2021artsheets,rostamzadeh2022healthsheet}, AI and data design guidelines~\cite{google2019pair}, ethical and societal impact statements at conferences~\cite{prunkl2021institutionalizing}, best practices for dataset management~\cite{mons2018data,jo2020lessons,hutchinson2021towards}, there is still a dearth of research understanding how fairness practitioners actually content with collecting new ``fairness-aware'' datasets. While it is clear from prior work that creating fairness-aware datasets come with a litany of challenges, it is currently unclear how the authors of fair datasets actually approach the processes of collection, annotation, and maintenance---or how they make decisions and tradeoffs during these processes.

% In this work we...
